Kimera-Multi: Robust, Distributed, Dense Metric-Semantic SLAM for Multi-Robot Systems

This paper presents Kimera-Multi, the first multi-robot system that (i) is robust and capable of identifying and rejecting incorrect inter and intra-robot loop closures resulting from perceptual aliasing, (ii) is fully distributed and only relies on local (peer-to-peer) communication to achieve distributed localization and mapping, and (iii) builds a globally consistent metric-semantic 3D mesh model of the environment in real-time, where faces of the mesh are annotated with semantic labels. Kimera-Multi is implemented by a team of robots equipped with visual-inertial sensors. Each robot builds a local trajectory estimate and a local mesh using Kimera. When communication is available, robots initiate a distributed place recognition and robust pose graph optimization protocol based on a novel distributed graduated non-convexity algorithm. The proposed protocol allows the robots to improve their local trajectory estimates by leveraging inter-robot loop closures while being robust to outliers. Finally, each robot uses its improved trajectory estimate to correct the local mesh using mesh deformation techniques. We demonstrate Kimera-Multi in photo-realistic simulations, SLAM benchmarking datasets, and challenging outdoor datasets collected using ground robots. Both real and simulated experiments involve long trajectories (e.g., up to 800 meters per robot). The experiments show that Kimera-Multi (i) outperforms the state of the art in terms of robustness and accuracy, (ii) achieves estimation errors comparable to a centralized SLAM system while being fully distributed, (iii) is parsimonious in terms of communication bandwidth, (iv) produces accurate metric-semantic 3D meshes, and (v) is modular and can be also used for standard 3D reconstruction (i.e., without semantic labels) or for trajectory estimation (i.e., without reconstructing a 3D mesh).

==> figures/diagram.tex <==
\begin{tikzpicture}[node distance = 40mm and 40mm, inner sep=5pt,thick,trim
		right=5cm,scale=0.5]
		%%%
		\tikzstyle{box}=[rectangle, very thick, draw, fill=#1, minimum
		width=12mm, minimum height=7mm, rounded corners=0.1cm]
		\tikzstyle{line} = [draw, -latex]
		\tikzstyle{dline} = [draw, latex-latex]
		%%%
		\node (images)        [box=white,align=center] {\footnotesize
		Stereo / Semantic / Depth Images};
		\node (imu)    		  [box=white,align=center,right= 1cm of images]
		{\footnotesize IMU};
		%\node (pointcloud)               [box=yellow!30,align=center,below= 1cm
		%of images,xshift=-2cm] {Convert to Point Cloud};
		%\node (denseStereoPointcloud)    [below= 1cm of pointcloud] {Dense Stereo Pointcloud};
		\node (semantics)                [box=blue!5,align=center,below= 0.5cm
		of images, xshift=-1cm] {\footnotesize Kimera Semantics};
		\node (incrementalMesh)          [below= 1cm of semantics,align=center]
		{\footnotesize Incremental\\\footnotesize Mesh};
		\node (pgmo)    	  			 [box=purple!40,align=center,below= 3.6cm of
		semantics] {\footnotesize Local Mesh Optimization};
		\node (vio)    	  [box=blue!4,align=center,below= 0.5cm of imu]
		{\footnotesize Kimera VIO};
		\node (bow)    	  [below= 0.4cm of vio,align=center] {\footnotesize BoW / 
		Descriptors / Keypoints};
		\node (lcd)    	  [box=orange!30,align=center,below= 0.35cm of bow,
		densely dashed, very thick] {\footnotesize Dist.\ Loop Closure Detection};
		\node (pcm)    	  [box=red!10,align=center,below= 0.35cm of lcd, densely
		dashed, very thick] {\footnotesize Dist.\ Outlier Rejection (PCM)};
		\node (dpgo)      [box=green!10,align=center,right= 2.31cm of pgmo,
		densely dashed, very thick] {\footnotesize Dist.\ PGO};
		\node (odometry)  [below= 0.45cm of vio, xshift=-3.1cm] {\footnotesize Odometry};
		\node (optimizedpg)  [left= 0.3cm of dpgo,align=center] {\footnotesize
		Optimized\\\footnotesize Pose Graph};
		%
		\node (optMesh)  [below= 0.7cm of pgmo,align=center] {\footnotesize
		Optimized Mesh};
		\node (optTraj)  [below= 0.7cm of dpgo,align=center] {\footnotesize Optimized Trajectory};
		%
		%\node (otherPcm)       [right= 1.5cm of pcm] {};
		%\node (otherDpgo)      [right= 1.5cm of dpgo] {};
		%\node (otherLcd)      [right= 1.5cm of lcd] {};
		%\node (other)      [above= 1.2cm of otherDpgo] {Other Robots};
		%
		%%%%%%%%%%%%%%%
		\path [line] (images) -- (semantics);
		\path [line] (images) -- (vio);
		%\path [line] (pointcloud) -- (denseStereoPointcloud);
		%\path [line] (denseStereoPointcloud) -- (semantics);
		\path [line] (semantics) -- (incrementalMesh);
		\path [line] (incrementalMesh) -- (pgmo);
		\path [line] (imu) -- (vio);
		\path [line] (vio) -- (odometry);
		\path [line] (vio) -- (bow);
		\path [line] (bow) -- (lcd);
		\path [line] (lcd) -- (pcm);
		\path [line] (pcm) -- (dpgo);
		\path [line] (odometry.south) |- (pcm);
		\path [line] (dpgo) -- (optimizedpg);
		\path [line] (optimizedpg) -- (pgmo);
		\path [line] (pgmo) -- (optMesh);
		\path [line] (dpgo) -- (optTraj);
%		\path [dline,dashed,thick] (dpgo) -- (otherDpgo);
%		\path [dline,dashed,thick] (pcm) -- (otherPcm);
%		\path [dline,dashed,thick] (lcd) -- (otherLcd);
		\draw [thick] ($(semantics.north west)+(-1.3,0.6)$)  rectangle
		($(dpgo.south east)+(2.5,-0.6)$);
		\draw [blue,very thick] ($(semantics.north west)+(-0.1,0.1)$)  rectangle	($(vio.south east)+(0.1,-0.1)$);
\end{tikzpicture}


